Fast Algorithm for K-Truss Discovery on Public-Private Graphs

In public-private graphs, users share one public graph and have their own private graphs. A private graph consists of personal private contacts that only can be visible to its owner, e.g., hidden friend lists on Facebook and secret following on Sina Weibo. However, existing public-private analytic algorithms have not yet investigated the dense subgraph discovery of k-truss, where each edge is contained in at least k-2 triangles. This paper aims at finding k-truss efficiently in public-private graphs. The core of our solution is a novel algorithm to update k-truss with node insertions. We develop a classification-based hybrid strategy of node insertions and edge insertions to incrementally compute k-truss in public-private graphs. Extensive experiments validate the superiority of our proposed algorithms against state-of-the-art methods on real-world datasets.

==> baseline.tex <==
In this section, we introduce two straight-forward algorithms for computing $k$-truss in public-private networks. 
One is an online search algorithm. The idea is intuitively simple. The algorithm first obtain the public-private ego-network and then apply truss decomposition on it for computing $k$-truss. 
The other method is to apply the truss updating algorithm with edge insertion on the graph $G_{N(v)}$ with new edges.
When there exists many edges to be inserted into graph $G$, the algorithm become very time consuming. To futher improve the efficiency, we propose a node-insertion algorithm for $k$-truss mining in public-private networks. 

\subsection{Brute-force Truss Decompostion}



% \begin{algorithm}[t]
% \small
% \caption{Truss Decomposition~\cite{WangC12} } 
% \label{algo:truss-decomp} 
% \begin{flushleft} 
% \textbf{Input:} $G=(V, E)$\\
% \textbf{Output:} $\tau(e)$ for each $e\in E$\\
% \end{flushleft}
% \vspace*{-0.3cm}
% \
% \begin{algorithmic}[1]

% \STATE Compute $sup_G(e)$ for each edge $e\in E$;

% \STATE Sort all the edges in ascending order of their support;

% \STATE $k \leftarrow 2$;

% \STATE \textbf{while} ($\exists e$ such that $sup_G(e) \leq (k-2)$)

% \STATE \hspace{0.3cm} Let $e=(u,v)$ be the edge with the lowest support;

% \STATE \hspace{0.3cm} Assume, w.l.o.g, $deg(u) \leq deg(v)$;

% \STATE \hspace{0.3cm} \textbf{for} (each $w\in N(u)$ \textbf{and} $(u,v)\in E$ \textbf{do})

% \STATE \hspace{0.6cm} $sup_G((u,w)) \leftarrow sup_G((u,w))-1$;

% \STATE \hspace{0.6cm} $sup_G((v,w)) \leftarrow sup_G((v,w))-1$;

% \STATE \hspace{0.6cm} Reorder $(u,w)$ and $(v,w)$ according to their new support;

% \STATE \hspace{0.3cm} $\tau_G(e) \leftarrow k$, remove $e$ from $G$;

% \STATE if(not all edges in $G$ are removed)

% \STATE \hspace{0.3cm} $k \leftarrow k+1$;

% \STATE \hspace{0.3cm} \textbf{Goto} Step 4;

% \STATE return $\{\tau_G(e)| e\in E\}$;

% \end{algorithmic}
% \end{algorithm}


\subsection{Edge-insertion Updating Algorithm}



